TA-RAG: Tone Awareness as a Design Imperative for Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) has become a robust architecture for grounding large language models (LLMs) in trusted knowledge. However, standard RAG systems exhibit a structural limitation: retrieved documents carry their own communication styles-professional jargon, formal tone, or academic writings-that shape the behavior of a RAG system before any tone instructions are processed, often causing the system to ignore user requests for a specific tone. We term this phenomenon contextual decoupling, in which a system optimises for factual accuracy while remaining decoupled from the social or operational context of the recipient. Building on prior research in public health peer-support communities, we identify three communicative misalignment-linguistic, cognitive, and relational-that can persist even when retrieval is relevant and the generated response is factually accurate. We conceptualise these as failures of communicative transformation, which remain largely invisible to accuracy-centred RAG evaluation metrics. To address this gap, we propose Tone-Aware RAG (TA-RAG), a conceptual architectural framework that positions communicative alignment alongside factual accuracy as a core design objective. TA-RAG operationalises four constraints-stigma-free language, readability alignment, recipient-sensitive adaptation, and empathetic framing-across the retrieval, context construction, generation, and constraint validation phases in the proposed RAG pipeline. We further highlight an evaluation agenda for jointly assessing factual fidelity and communicative alignment, and identify open challenges. We argue that tone awareness should be treated not as an optional refinement, but as a present design imperative for RAG systems operating in socially sensitive and high-stakes contexts.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

The computing community has invested significant effort in improving factual grounding in generative systems. Yet, communicative misalignment remains a potent source of harm and distrust. In RAG systems, this misalignment arises from the interaction between retrieved content and generation, where implicit communicative norms are reproduced without regard to user context.
Tone-awareness is therefore not an aesthetic refinement but a communicative responsibility. In domains such as healthcare, education, and human-AI interaction, the manner in which information is conveyed—its framing, accessibility, and affective alignment—shapes comprehension, engagement, and trust as strongly as the content itself. Addressing this gap requires moving beyond accuracy-centric design toward systems that explicitly model communication as part of their core functionality.
We conceptualise TA-RAG as a framework for operationalising this shift. By embedding stigma-free language constraints, readability control, recipient adaptation, and affective alignment as system-level components, TA-RAG transforms tone from an incidental outcome into an enforceable property in the RAG pipeline. This enables systematic evaluation and improvement of communicative alignment in AI-mediated systems.
The central question for the computing community is no longer only whether systems can retrieve accurate information, but whether they can deliver it in ways that sustain trust, respect user context, and support meaningful interaction.
Looking forward, integrating tone-awareness into RAG systems introduces several research challenges. These include the development of tone-aware retrieval strategies that account for communicative norms in source selection, robust evaluation metrics for assessing communicative alignment, and human-in-the-loop validation frameworks that reflect domain-specific expectations. More broadly, this shift reframes RAG not merely as an informational architecture, but as a communicative system embedded in social contexts. Addressing this challenge will be critical to ensuring that AI systems not only inform, but communicate responsibly.
